High-performance Kernel Machines with Implicit Distributed Optimization and Randomization

In order to fully utilize "big data", it is often required to use "big models". Such models tend to grow with the complexity and size of the training data, and do not make strong parametric assumptions upfront on the nature of the underlying statistical dependencies. Kernel methods fit this need well, as they constitute a versatile and principled statistical methodology for solving a wide range of non-parametric modelling problems. However, their high computational costs (in storage and time) pose a significant barrier to their widespread adoption in big data applications. We propose an algorithmic framework and high-performance implementation for massive-scale training of kernel-based statistical models, based on combining two key technical ingredients: (i) distributed general purpose convex optimization, and (ii) the use of randomization to improve the scalability of kernel methods. Our approach is based on a block-splitting variant of the Alternating Directions Method of Multipliers, carefully reconfigured to handle very large random feature matrices, while exploiting hybrid parallelism typically found in modern clusters of multicore machines. Our implementation supports a variety of statistical learning tasks by enabling several loss functions, regularization schemes, kernels, and layers of randomized approximations for both dense and sparse datasets, in a highly extensible framework. We evaluate the ability of our framework to learn models on data from applications, and provide a comparison against existing sequential and parallel libraries.

==> implementation.tex <==
\section{Implementation}

Elemental/OpenMP

==> problem.tex <==
\section{Problem Definition}

Let $\vv{X}\in \reals^{n \times d}$ be a data matrix where
$n$ is the number of examples and $d$ is the number of features. We assume that
$n$ is very large relative to $d$. The corresponding multiple labels are arranged in a matrix $\vv{Y} \in \reals^{n\times k}$ where $k$ is the number of classes or targets. Associated with $\vv{X}$ is a matrix $\vv{Z}\in \reals^{n\times s}$
which we call the feature space data matrix obtained through an explicit
feature mapping associated with a kernel function. The dimensionality $s$ can
also be very large. The transpose of the corresponding rows of $\vv{X}, \vv{Y}$ and $\vv{Z}$, treated as column vectors, will be denoted as $\vv{x}_i, \vv{y}_i$ and $\vv{z}(\vv{x}_i)$ respectively. We are interested in large-scale distributed convex optimization for solving
regularized risk minimization problems of the form,

\begin{equation}
\argmin_{\vv{W}\in \reals^{s\times k}} \frac{1}{n} \sum_{i=1}^n V\left(
\vv{y}_i, \vv{W}^T \vv{z}(\vv{x}_i)\right) + \lambda r(\vv{W}) \label{eq:problem_linear}
%\end{equation} where $V(\cdot, \cdot)$ is a convex loss function, $r$ is a convex regularizer, $\lambda\geq 0$ is a regularization parameter and $\vv{W}$ contains the  coefficients or weights of a multivariate linear model. Though our framework is highly generalizable, for concreteness we will  focus on $l_2$ regularization i.e. $r(\vv{W}) = \|\vv{W}\|^2_{fro}$, and the following choices of the loss function.
%
%\begin{table}[h]
%\small{
%\caption{Loss functions}
%\begin{tabular}{ccc}
%\hline
%Loss & $V(\vv{y}, \vv{o})$ & $\y$ domain\\
%\hline 
%\textrm{Squared} & $\frac{1}{2} \|\vv{o} - \vv{y}\|^2$ & $\vv{y}\in \reals^k$~~~~~~~ \\ 
%$l_1$ & $\frac{1}{2} \|\vv{y} - \vv{o}\|_1$ &  $\vv{y}\in \reals^k$~~~~~~~~\\ 
%\textrm{Hinge} &  $\sum_{i=1}^k \max\left(0, 1 - y_i o_i\right)$ &  $\vv{y}\in \{+1,-1\}^k$  \\
%\textrm{Multinomial Logistic} & $o_{\vv{y}} - \log \sum_{i=1}^k e^{o_i}$  & $\vv{y}\in \{1\ldots k\}$ \\
\hline
\end{tabular}
}
\end{table}
 
The prox operators for these loss f

==> randkernels.tex <==
\section{Randomized Algorithms for Kernel Methods}












